How to Leverage Unlabeled Data in Offline Reinforcement Learning

Offline reinforcement learning (RL) can learn control policies from static datasets but, like standard RL methods, it requires reward annotations for every transition. In many cases, labeling large datasets with rewards may be costly, especially if those rewards must be provided by human labelers, while collecting diverse unlabeled data might be comparatively inexpensive. How can we best leverage such unlabeled data in offline RL? One natural solution is to learn a reward function from the labeled data and use it to label the unlabeled data. In this paper, we find that, perhaps surprisingly, a much simpler method that simply applies zero rewards to unlabeled data leads to effective data sharing both in theory and in practice, without learning any reward model at all. While this approach might seem strange (and incorrect) at first, we provide extensive theoretical and empirical analysis that illustrates how it trades off reward bias, sample complexity and distributional shift, often leading to good results. We characterize conditions under which this simple strategy is effective, and further show that extending it with a simple reweighting approach can further alleviate the bias introduced by using incorrect reward labels. Our empirical evaluation confirms these findings in simulated robotic locomotion, navigation, and manipulation settings.

==> UDS_ICML_camera_ready_arXiv 2/defs.tex <==
\newcommand{\cmt}[1]{{\footnotesize\textcolor{red}{#1}}}
\newcommand{\cmto}[1]{{\footnotesize\textcolor{orange}{#1}}}
\newcommand{\note}[1]{\cmt{Note: #1}}
\newcommand{\question}[1]{\cmto{Question: #1}}
\newcommand{\sergey}[1]{{\footnotesize\textcolor{blue}{Sergey: #1}}}
\newcommand{\ak}[1]{{\textcolor{black}{#1}}}
\newcommand{\edits}[1]{\textcolor{blue}{#1}}
\newcommand{\editsred}[1]{\textcolor{red}{#1}}
\newcommand{\editsp}[1]{\textcolor{purple}{#1}}
\newcommand{\editsv}[1]{\textcolor{magenta}{#1}}



\newcommand{\x}{\mathbf{x}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\data}{\mathcal{D}}

\newcommand{\etal}{{et~al.}\ }
\newcommand{\eg}{\emph{e.g.},\ }
\newcommand{\ie}{\emph{i.e.},\ }
\newcommand{\nth}{\text{th}}
\newcommand{\pr}{^\prime}
\newcommand{\tr}{^\mathrm{T}}
\newcommand{\inv}{^{-1}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\gauss}{\mathcal{N}}
\newcommand{\norm}[1]{\left|#1\right|}
\newcommand{\trace}{\text{tr}}

\newcommand{\reward}{r}
\newcommand{\policy}{\pi}
\newcommand{\mdp}{\mathcal{M}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\actions}{\mathcal{A}}
\newcommand{\observations}{\mathcal{O}}
\newcommand{\transitions}{T}
\newcommand{\initstate}{d_0}
\newcommand{\freq}{d}
\newcommand{\obsfunc}{E}
\newcommand{\initial}{\mathcal{I}}
\newcommand{\horizon}{H}
\newcommand{\rewardevent}{R}
\newcommand{\probr}{p_\rewardevent}
\newcommand{\metareward}{\bar{\reward}}
\newcommand{\discount}{\gamma}
\newcommand{\behavior}{{\pi_\beta}}
\newcommand{\bellman}{\mathcal{B}}
\newcommand{\qparams}{\phi}
\newcommand{\qparamset}{\Phi}
\newcommand{\qset}{\mathcal{Q}}
\newcommand{\batch}{B}
\newcommand{\qfeat}{\mathbf{f}}
\newcommand{\Qfeat}{\mathbf{F}}
\newcommand{\hatbehavior}{\hat{\pi}_\beta}

\newcommand{\traj}{\tau}

\newcommand{\pihi}{\pi^{\text{hi}}}
\newcommand{\pilo}{\pi^{\text{lo}}}
\newcommand{\ah}{\mathbf{w}}

\newcommand{\proj}{\Pi}

\newcommand{\loss}{\mathcal{L}}
\newcommand{\eye}{\mathbf{I}}

\newcommand{\model}{\hat{p}}

\newcommand{\pimix}{\pi_{\text{mix}}}

\newcommand{\pib}{\bar{\pi}}
\newcommand{\epspi}{\epsilon_{\pi}}
\newcommand{\epsmodel}{\epsilon_{m}}

\newcommand{\return}{\mathcal{R}}

\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\en}{\mathcal{E}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\boldm}{\mathbf{m}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\ot}{\bo_t}
\newcommand{\st}{\bs_t}
\newcommand{\at}{\ba_t}
\newcommand{\op}{\mathcal{O}}
\newcommand{\opt}{\op_t}
\newcommand{\kl}{D_\text{KL}}
\newcommand{\tv}{D_\text{TV}}
\newcommand{\ent}{\mathcal{H}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\byk}{\mathbf{y_k}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bO}{\mathbf{O}}

\newcommand{\bzhi}{\bz^\text{hi}}
\newcommand{\expected}{\mathbb{E}}
\newcommand{\srank}{\text{srank}}
\newcommand{\rank}{\text{rank}}
\newcommand{\deepnet}{\bW_N(k, t) \bW_\phi(k, t)}
\newcommand{\features}{\bW_\phi(k, t)}
\newcommand{\stateactioni}{[\bs_i; \ba_i]}
\newcommand{\diag}{\text{\textbf{diag}}}
\newcommand{\cosine}{\text{cos}}
\newcommand{\indicator}{\mathds{1}}


\def\thetaP{\theta^{\prime}}
\def\cf{\emph{c.f.}\ }
\def\vs{\emph{vs}.\ }
\def\etc{\emph{etc.}\ }
\def\Eqref#1{Equation~\ref{#1}}

\newenvironment{repeatedthm}[1]{\@begintheorem{#1}{\unskip}}{\@endtheorem}

\newcommand{\methodname}{CDS}
\newcommand{\aliasingproblemname}{bootstrapping aliasing}
\newcommand{\Aliasingproblemname}{Bootstrapping aliasing}
\newcommand{\AliasingProblemName}{Bootstrapping Aliasing}
\newcommand{\simnorm}{\mathrm{sim}_{\mathrm{n}}^\pi}
\newcommand{\simunnorm}{\mathrm{sim}_{\mathrm{u}}^\pi}
\newcommand{\uds}{UDS}

==> UDS_ICML_camera_ready_arXiv 2/experiments.tex <==

\section{Experiments}
\label{sec:exp}
In our experiments, we aim to evaluate whether the theoretical potential for simple minimum-reward relabeling to attain good results is reflected in benchmark tasks and more complex offline RL settings. In particular, we will study: \textbf{(1)} can UDS match or exceed the performance of sophisticated reward inference methods and methods with oracle reward functions in simulated locomotion and navigation tasks? \textbf{(2)} can an optimized reweighting strategy (e.g., CDS+UDS) further improve the results achieved by UDS?, \textbf{(3)} how does UDS behave with and without combining with an optimized reweighting strategy in multi-task offline RL settings?, \textbf{(4)} under which conditions does UDS work and not work and does optimizing for reweighting help?

\begin{table*}[ht]
\vspace{-0.2cm}
\caption{\footnotesize Results for multi-task robotic manipulation (Meta-World) and navigation environments (AntMaze) with low-dimensional state inputs. Numbers are averaged across 6 seeds, $\pm$ the 95$\%$-confidence interval. We take the results of No Sharing, Sharing All and CDS, directly from \cite{yu2021conservative}. We bold the best-performing method that does not have access to the true rewards for relabeling. We include per-task performance for Meta-World domains and the overall performance averaged across tasks (highlighted in gray) for all three domains. Both CDS+UDS and UDS outperforms prior vanilla multi-task offline RL approach (No Sharing) and reward learning methods (Reward Predictor, VICE and RCE) while performing competitively compared to oracle reward relabeling methods.}
\begin{center}
\resizebox{\textwidth}{!}{\begin{tabular}{l|l|rrrrrr|rr}
\toprule
& & & & & & & & \multicolumn{2}{c}{\textbf{Oracle Methods}} \\
\textbf{Environment} & \textbf{Tasks} & \textbf{CDS+UDS} & \textbf{UDS} & \textbf{VICE} & \textbf{RCE} & \textbf{No Sharing} & \textbf{Reward Pred.} & \textbf{CDS} & \textbf{Sharing All}\\ \midrule
& door open & \textbf{61.3\%}$\pm$7.9\% & 51.9\%$\pm$25.3\% & 0.0\%$\pm$0.0\% & 0.0\%$\pm$0.0\% & 14.5\%$\pm$12.7\% & 0.0\%$\pm$0.0\% & 58.4\%$\pm$9.3\% & 34.3\%$\pm$17.9\%\\
& door close & 54.0\% $\pm$42.5\% & 12.3\%$\pm$27.6\% & 66.7\%\%$\pm$47.1\% & 0.0\%$\pm$0.0\% & 4.0\%$\pm$6.1\% & \textbf{99.3\%}$\pm$0.9\% & 65.3\%$\pm$27.7\% & 48.3\%$\pm$27.3\%\\
Meta-World& drawer open & \textbf{73.5\%}$\pm$9.6\% & 61.8\%$\pm$16.3\% & 0.0\%$\pm$0.0\% & 0.0\%$\pm$0.0\% & 16.0\%$\pm$17.5\% & 13.3\%$\pm$18.9\% & 57.9\%$\pm$16.2\% & 55.1\%$\pm$9.4\%\\
& drawer close & 99.3\%$\pm$0.7\% & \textbf{99.6\%}$\pm$0.7\% & 19.3\%$\pm$27.3\% & 2.7\%$\pm$1.7\% & 99.0\%$\pm$0.7\% & 50.3\%$\pm$35.8\% & 99.0\%$\pm$0.7\% & 98.8\%$\pm$0.7\%\\
& \CC \textbf{average} & \CC \textbf{71.2\%} $\pm$ 11.3\% & \CC 56.4\%$\pm$12.8\% & \CC 21.5\%$\pm$0.7\% & \CC 0.7\%$\pm$0.4\% & \CC 33.4\%$\pm$8.3\% & \CC 41.0\%$\pm$11.9\% & \CC 70.1\%$\pm$8.1\% & \CC 59.4\%$\pm$5.7\%\\
\midrule
AntMaze    & medium (3 tasks)  &\textbf{31.5\%}$\pm$3.0\% & 26.5\%$\pm$9.1\%  & 2.9\%$\pm$1.0\%  & 0.0\%$\pm$0.0\%  & 21.6\%$\pm$7.1\% & 3.8\%$\pm$3.8\% & 36.7\%$\pm$6.2\%  & 22.9\%$\pm$3.6\%\\
& large (7 tasks)  & \textbf{18.4\%}$\pm$6.1\% & 14.2\%$\pm$3.9\% & 2.5\%$\pm$1.1\% & 0.0\%$\pm$0.0\% & 13.3\% $\pm$ 8.6\% & 5.9\%$\pm$4.1\% & 22.8\% $\pm$ 4.5\% & 16.7\% $\pm$ 7.0\%\\
\bottomrule
\end{tabular}}
\end{center}
\vspace{-0.3cm}
\label{tbl:gym}
\normalsize
\end{table*}


\begin{table*}[ht]
\vspace*{-0.3cm}
\caption{\footnotesize Results for multi-task imaged-based robotic manipulation domains in \citep{yu2021conservative}. Numbers are averaged across 3 seeds, $\pm$ the 95$\%$ confidence interval. UDS outperforms No Sharing in 7 out of 10 tasks as well as the average task performance, while performing comparably to Sharing All. CDS+UDS further improves the performance of UDS and outperforms No Sharing in all of the 10 tasks.
}
\small{
\begin{center}
\begin{tabular}{l|rrr|rr}
\toprule
\textbf{Task Name} & \textbf{CDS+UDS}& \textbf{UDS} & \textbf{No Sharing} & \textbf{CDS (oracle)} & \textbf{Sharing All (oracle)}\\ \midrule
\texttt{lift-banana} & \textbf{55.9\%}$\pm$11.7\% & 48.6\%$\pm$5.1\% & 20.0\%$\pm$6.0\% &  \textbf{53.1\%}$\pm$3.2\% & 41.8\%$\pm$4.2\%\\
\texttt{lift-bottle} & \textbf{72.9\%}$\pm$12.8\% & 58.1\%$\pm$3.6\%& 49.7\%$\pm$8.7\% & \textbf{74.0\%}$\pm$6.3\% & 60.1\%$\pm$10.2\%\\
\texttt{lift-sausage} & \textbf{74.3\%}$\pm$8.3\%  & 66.8\% $\pm$ 2.7\%  & 60.9\%$\pm$6.6\% & \textbf{71.8\%}$\pm$3.9\% & 70.0\%$\pm$7.0\%\\
\texttt{lift-milk}& 73.5\%$\pm$6.7\% & \textbf{74.5\%}$\pm$2.5\% & 68.4\%$\pm$6.1\% & \textbf{83.4\%}$\pm$5.2\% & 72.5\%$\pm$5.3\%\\

\texttt{lift-food} & \textbf{66.3\%}$\pm$8.3\% & 53.8\%$\pm$8.8\%  & 39.1\%$\pm$7.0\% & \textbf{61.4\%}$\pm$9.5\% & 58.5\%$\pm$7.0\%\\
\texttt{lift-can} & \textbf{64.9\%}$\pm$7.1\%  & 61.0\%$\pm$6.8\%  & 49.1\%$\pm$9.8\% & \textbf{65.5\%}$\pm$6.9\% & 57.7\%$\pm$7.2\%\\
\texttt{lift-carrot} & \textbf{84.1\%}$\pm$3.6\% & 73.4\%$\pm$5.8\% & 69.4\%$\pm$7.6\% & \textbf{83.8\%}$\pm$3.5\% & 75.2\%$\pm$7.6\%\\
\texttt{place-bowl} & \textbf{83.4\%}$\pm$3.6\%  & 77.6\%$\pm$1.6\%  & 80.3\%$\pm$8.6\% & \textbf{81.0\%}$\pm$8.1\% & 70.8\%$\pm$7.8\%\\
\texttt{place-plate} & \textbf{86.2\%}$\pm$1.8\%  & 78.7\%$\pm$2.2\%  & 86.1\%$\pm$7.7\% & \textbf{85.8\%}$\pm$6.6\% & 78.7\%$\pm$7.6\%\\
\texttt{place-divider-plate} & \textbf{89.0\%}$\pm$2.2\%  & 80.2\%$\pm$2.2\%  & 85.0\%$\pm$5.9\% & \textbf{87.8\%}$\pm$7.6\% & 79.2\%$\pm$6.3\%\\
\CC \textbf{average} & \CC \textbf{75.0\%}$\pm$3.3\%  & \CC 67.3\%$\pm$0.8\% & \CC 60.8\%$\pm$7.5\% & \CC \textbf{74.8\%} $\pm$6.4\% & \CC 66.4\%$\pm$7.2\%\\
\bottomrule
\end{tabular}
\end{center}
\vspace{-0.7cm}
\label{tbl:mtopt}
}
\end{table*}

\textbf{Comparisons.} 
We evaluate multiple approaches alongside with \textbf{UDS} and \textbf{CDS+UDS}:
\textbf{No Sharing}, which uses the labeled data only without using any of the unlabeled data, \textbf{Reward Predictor}, which is trained via supervised classification or regression to directly predict the reward in sparse and dense reward settings respectively, \textbf{VICE}~\citep{fu2018variational} and \textbf{RCE}~\citep{eysenbach2021replacing}, inverse RL methods only applicable to sparse reward settings, that learn either a reward or Q-function classifier from both the labeled data and unlabeled data (treated as negatives) and then annotate the unlabeled data with the learned classifier, 
In the multi-task setting, we modify \textbf{VICE} and \textbf{RCE} accordingly by extracting transitions with reward labels equal to 1 and treating these datapoints as positives to learn the classifier for each task. We also train \textbf{No Sharing}, \textbf{Reward Predictor}, \textbf{VICE} and \textbf{RCE}, but adapt them to the offline setting using CQL, i.e. the same underlying offline RL method as in \textbf{UDS} and \textbf{CDS+UDS}.
For more details on experimental set-up and hyperparameter settings, please see Appendix~\ref{app:details}. 
\rebuttal{We also include evaluations of our methods under different quality of the relabeled data in Appendix~\ref{app:data_quality} and comparisons to model-based offline RL approaches in Appendix~\ref{app:mbrl} and prior methods~\citep{yang2021representation,yang2021trail} that leverage unlabeled data for representation learning instead of sharing directly in Appendix~\ref{app:pretrained_reps}.}

\textbf{Datasets and tasks.} To answer questions (1) and (2), we perform empirical evaluations on two state-based single-task locomotion datasets. To answer question (3), we further evaluate all methods on three state-based multi-task datasets that consist of robotic manipulation, navigation and locomotion domains respectively and one image-based multi-task manipulation dataset from prior work \citep{yu2021conservative}.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.35\textwidth]{env.png}
    \vspace{-0.33cm}
    \caption{\footnotesize  Environments (from left to right):  single-task hopper, single-task and multi-task AntMaze, multi-task walker, multi-task Meta-World, and multi-task vision-based pick-place tasks.}
    \vspace{-0.35cm}
    \label{fig:env}
\end{figure}

\noindent \textbf{Single-task domains \& datasets.} We adopt two environments: hopper and the AntMaze from the D4RL benchmark~\citep{fu2020d4rl} for evaluation in the single-task setting. For the hopper environment, we consider two scenarios where we have 10k labeled data from the {hopper-expert} and 1M unlabeled transitions from the {hopper-random} datasets and {hopper-medium} datasets respectively. This setup is resembles practical problems where unlabeled data is of low-quality and even, irrelevant to the target task.
For AntMaze, following the setup in \cite{yang2021trail}, we use 10k expert transitions as the labeled data and the entire datasets of {large-play} and {medium-play} as the unlabeled data.


\begin{table*}[ht]
\vspace{-0.3cm}
\caption{\footnotesize We perform an empirical analysis on the single-task environment \texttt{hopper} from D4RL~\citep{fu2020d4rl} benchmark to test the sensitivity of UDS under the data quality and data coverage for both the labeled task data and unlabeled data. The numbers are averaged over \final{ten} random seeds. We bold the best method without true reward relabeling. UDS outperforms No Sharing in 5 out of 6 settings while achieving competitive performances compared to Sharing All in 5 out of 6 settings.
CDS+UDS is able to further improve over UDS significantly in such a setting and also outperforms UDS in 5 out of 6 settings in general.
}
\vspace{-0.3cm}
\begin{center}
\resizebox{\textwidth}{!}{\begin{tabular}{l|l|l|rrr|rr}
\toprule
& & & & & & \multicolumn{2}{c}{\textbf{Oracle Methods}} \\
 \textbf{Environment} & \textbf{Labeled data type / size} & \textbf{Unlabeled data type / size}   & \textbf{CDS+UDS}   & \textbf{UDS}         & \textbf{No Sharing} & \textbf{CDS} & \textbf{Sharing All} \\
 \midrule
& \textbf{(a)} expert / 10k transitions & random / 1M transitions & \textbf{82.1}  & 78.8 & 77.1 & 83.3 & 86.1\\
& \textbf{(b)} expert / 10k transitions & medium / 1M transitions   & \textbf{78.1} & 64.8 & 77.1 & 82.5 & 64.6\\
& \textbf{(c)} expert / 10k transitions & expert / 990k transitions   & 106.1 & \textbf{108.4} & 77.1 & 106.6 & 112.3\\
 D4RL hopper  & \textbf{(d)} medium / 10k transitions & random / 1M transitions & \textbf{33.2}  & 9.9 & 28.7 & 41.2 & 38.9\\
& \textbf{(e)} medium / 10k transitions & expert / 1M transitions & \textbf{108.9}   & 106.7 & 28.7 & 111.1 & 107.5\\
& \textbf{(f)} random / 10k transitions & medium / 1M transitions & \textbf{63.5}  & 47.1 & 9.6 & 92.3 & 69.8\\
& \textbf{(g)} random / 10k transitions & expert / 1M transitions  & \textbf{101.2} & 95.9 & 9.6 & 110.9 & 102.8\\
\bottomrule
\end{tabular}}
\end{center}
\vspace{-0.7cm}
\label{tbl:single_task_analysis}
\normalsize
\end{table*}

\noindent \textbf{Multi-task domains \& datasets.} We consider several multi-task domains. The first set of domains are from prior work~\citep{yu2021conservative}: \textbf{(i)} the Meta-World~\citep{yu2020meta} domain, which consists of four tasks of opening and closing doors and drawers; and \textbf{(ii)} the Antmaze~\citep{fu2020d4rl} domain, which consists of mazes of two sizes (medium and large) with 3 and 7 tasks corresponding to different goal positions respectively. We also evaluate on the multi-task walker environment with dense rewards, which we will discuss in detail in Appendix~\ref{app:dense_reward}.
In addition, we test multi-task offline RL methods with UDS in the multi-task visual manipulation domain, which provides a realistic scenario, of the sorts we will encounter in robotic settings in practice. In this domain, there are 10 tasks with different combinations of object-oriented grasping, with 7 objects (banana, bottle, sausage, milk box, food box, can and carrot), as well as placing the picked objects onto one of three fixtures (bowl, plate and divider plate). For domains except the walker environment, we use binary rewards, where $1$ denotes the successful completion of the task and $0$ corresponds to failure. We also use the datasets used in \cite{yu2021conservative} for all domains. For details, see Appendix~\ref{app:env_data_details}.


\vspace{-0.1cm}
\subsection{Results of Empirical Evaluations}
\label{sec:results}
\vspace{-0.1cm}
\noindent \textbf{Results of Question (1) and (2).} We evaluate each method on the single-task hopper and AntMaze domains. As shown in Table~\ref{tbl:single_task}, we find that UDS outperforms No Sharing in 3 out of the 4 settings and reward learning methods in all the settings. We hypothesize that reward learning methods underperform because reward predictors are unable to achieve reasonable generalization ability in the limited labeled data setting. Note that UDS even achieves competitive performance as the oracle Sharing All method. Furthermore, an optimized reweighting scheme, i.e., CDS+UDS, is able to improve over UDS in each case, including cases where UDS fails to improve over No Sharing, indicating a large reward bias. These results testify to the effectiveness of optimizing for reweighting when dealing with unlabeled data. Note that on the AntMaze domain, CDS+UDS performs comparably to the recent approach~\citep{yang2021trail} that performs representation learning on the offline dataset first and then run offline training leveraging the learned representation. CDS+UDS also outperforms all the prior methods in offline training with learned representations discussed in \cite{yang2021trail}.

\noindent \textbf{Results of Question (3).} Observe in Table~\ref{tbl:gym} that UDS outperforms na\"ive multi-task offline RL without data sharing and reward learning methods, suggesting that leveraging unlabeled data with our simple method UDS can boost offline RL performance in both multi-task manipulation and navigation domains.
Since reward learning approaches obtain similar or worse results compared to No Sharing, which we suspect could be due to erroneous predictions on unseen transitions in the multi-task data, we only compare our methods to No Sharing and the oracle methods in the image-based experiments. As shown in Table~\ref{tbl:mtopt}, UDS outperforms No Sharing in 7 out of 10 tasks as well as the average task performance by a significant margin. Therefore, UDS is able to effectively leverage unlabeled data from other tasks and achieves potentially surprisingly strong results compared to more sophisticated methods that handle unlabeled offline data. We also find that CDS+UDS further improves upon the performance of UDS, which indicates that optimizing for reweighting via CDS+UDS can actually work well.




Finally, note that, CDS+UDS and UDS attain performance competitive with their oracle counterparts, CDS and Sharing All, that assume access to full reward information, both in Tables~\ref{tbl:gym} \& \ref{tbl:mtopt}. This is potentially very surprising, and one could hypothesize that this might be because most transitions in the unlabeled dataset were actually failures, and hence, were labeled correctly by UDS. However, to the contrary, our diagnostic analysis in Table~\ref{tbl:data_quality}, Appendix~\ref{app:data_quality} reveals that the unlabeled data \emph{does not} consist entirely of failures; in fact, around 60\% of the unlabeled data succeeds at the task of interest, indicating that the rewards are wrong for more than half the unlabeled data. In spite of this, UDS and CDS+UDS perform well. This indicates that the simple UDS approach can be effective in removing the dependence of functional form of reward functions, which is often costly, without much loss in the performance and CDS+UDS can boost performance by reducing the bias.





\subsection{Empirical Analysis of UDS and CDS+UDS}
\label{sec:empirical_analysis}

To answer question (4), we analyze UDS and CDS+UDS on several offline RL problems designed to test robustness and sensitivity to the data coverage and the data quality on the single-task hopper domain. To create these instances, we consider 7 different combinations of data quality ({hopper-expert}, {hopper-medium} or {hopper-random}) and amount of labeled and unlabeled data labeled as \textbf{(a)}-\textbf{(g)} in Table~\ref{tbl:single_task_analysis}. In Appendix~\ref{app:mw_analysis}, we present results for a similar analysis in the multi-task Meta-World setting. We evaluate UDS, CDS+UDS and No Sharing in each case, and also present results for CDS and Sharing All approaches which assume access to the actual reward, for understanding. \final{Additionally, we conduct an ablation that compares UDS and CDS+UDS to reward learning methods in settings where the labeled data size and quality are varied, which is included in Appendix~\ref{app:reward_learning_ablation}.}


When the labeled data is of expert-level, adding unlabeled random or medium data (cases \textbf{a} and \textbf{b} in Table~\ref{tbl:single_task_analysis}) should only increase coverage, since the labeled data only consists of expert transitions. Moreover, the reward bias induced due to incorrect labeling of rewards on the medium unlabeled data should not hurt, since the 10k expert transitions retain their correct labels, and the medium/random data should only serve as negatives, provided the annotated rewards on this data are worse than the rewards in the expert data. Therefore, we expect the benefits of coverage to outweigh any reward bias; as seen in Table~\ref{tbl:single_task_analysis}, we find that UDS indeed helps compared to No Sharing. In particular, in those two cases, UDS approaches the oracle Sharing All method. 

Since reward bias is exacerbated when the unlabeled data is of higher quality and present in large amounts (cases \textbf{e, f, g}), it is reasonable to surmise that UDS will perform worse in such scenarios. However, on the contrary, in settings: random labeled data with medium or expert unlabeled data and medium labeled data with expert unlabeled data, we find that even though the rewards on the unlabeled transitions are incorrect, the addition of unlabeled data into training improves performance. This is because a higher quality unlabeled data improves the performance of the effective behavior policy, thereby improving performance for a conservative offline RL method. This result validates Theorem~\ref{prop:uds_ours}. 
We also conduct an ablation that varies the amount of unlabeled data in Appendix~\ref{app:unlabeled_dataset_size_analysis}. This ablation shows that the benefit of UDS reduces as the we reduce the amount of unlabeled data, which confirms our theory in Section~\ref{sec:uds_theory}.

In the case where labeled data is medium and unlabeled data is random (case \textbf{d}), we find that UDS hurts compared to No Sharing. This is because the labeled data as well as unlabeled data are both low-medium quality and medium data already provides decent coverage (not as high as random data, but not as low as expert data). Therefore, in this case, we believe that the addition of unlabeled data neither provides trajectories of good quality that can help improve performance, nor does it significantly improve coverage, and only hurts by incurring reward bias. We therefore believe that UDS may not help in such cases where the coverage does not improve, and added data is not so high quality, which also agrees with our theoretical analysis. Furthermore, in the case where the labeled and unlabeled data are both expert (case \textbf{c}), UDS performs close to oracle methods CDS and Sharing All, which confirms the insights derived from Section~\ref{sec:uds_theory} that UDS does not introduce bias when the labeled and unlabeled data have the same distribution and hence should perform well.

Finally, note that CDS+UDS is able to improve over UDS in 5 out of 6 settings in hopper, suggesting that CDS+UDS gains benefit from reducing the reward bias as well as the sampling error shown in Section~\ref{sec:method}.





==> UDS_ICML_camera_ready_arXiv 2/intro.tex <==
\section{Introduction}

==> UDS_ICML_camera_ready_arXiv 2/math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> UDS_ICML_camera_ready_arXiv 2/method.tex <==
\section{How To Use Unlabeled Data in Offline RL}
\vspace{-0.1cm}
\label{sec:method}
Arguably the easiest approach to utilize unlabeled data in offline RL is to simply assign the lowest possible reward to all the transitions in the unlabeled data, which we will assume to be $0$ without loss of generality, and use this data for training the underlying offline RL method. We will refer to this approach as UDS. We will show that, although this strategy might seem simplistic, in fact, it can work well both in theory and practice, when the dataset composition and the task satisfies certain criteria. Not all tasks and datasets satisfy these criteria, but we will argue that many realistic offline RL problems do satisfy them. For example, UDS can work well in a problem where the labeled data consists of high-quality, near-expert demonstrations, while the unlabeled data consists of mediocre or low-reward interactions in the environment, as is often the case in robotics~\citep{xie2019improvisation}. 
We will analyze the performance of this approach theoretically in Section~\ref{sec:uds_theory} and empirically in Section \ref{sec:empirical_analysis}.

Although the simple UDS approach can perform well in some scenarios, relabeling with zero reward of course also biases the learning process. We therefore further show that reward bias can be mitigated if the unlabeled transitions are additionally reweighted, so as to change the unlabeled data distribution (while still using a label of zero for all unlabeled data). While such reweighting reduces the sample size, it can provide an overall benefit by reducing the reward bias \ak{and distributional shift}. We will derive the optimal scheme for reweighting the transitions in the unlabeled dataset that minimizes the impact of reward bias in Section~\ref{sec:rebalancing}. Surprisingly, our analysis reveals that a near-optimal solution to reducing reward bias is to combine \uds\ with an already existing reweighting scheme for multi-task offline RL with full reward information. For example, one can choose to reweight unlabeled data with the  {CDS} scheme of \citet{yu2021conservative}, which preferentially upweights transitions based on their conservative Q-values.

\vspace{-0.1cm}
\subsection{Theoretical Analysis of UDS in Offline RL}
\vspace{-0.1cm}
\label{sec:uds_theory}
In this section, we will derive a performance bounds for \uds\ that allow us to understand several cases when this simple baseline approach still works well. We will show that the increase in the effective dataset size can often outweigh the bias incurred from using the wrong reward in several practical situations. We will also discuss conditions on the data composition and the relative distributions of labeled and unlabeled data that enable UDS to be successful.
Formally, UDS trains on an effective dataset given by:
\begin{equation}
    \mathcal{D}^\mathrm{eff} = \mathcal{D}_\mathrm{L} \cup \{(\bs_j, \ba_j, \bs'_j, 0) \in \mathcal{D}_{\mathrm{U}}\}. \label{eq:uds}
\end{equation}
We now present a policy improvement guarantee for UDS below, and then analyze the bound under special conditions. Our theoretical result builds on techniques for showing safe policy improvement bounds~\citep{laroche2019safe,kumar2020conservative,yu2021conservative}. 

\begin{table*}[t]
\vspace{-0.15cm}
\caption{\footnotesize Summary of scenarios where UDS is expected to work and where it is not expected to work. \textbf{L} denotes the characteristics of labeled data, \textbf{U} denotes characteristics of unlabeled data. Limited/Abundant refers to the relative amount of data available
High-quality/medium-quality/low-quality refers to the actual performance of the behavior policy generating the datasets. Narrow/broad refers to the relative state coverage of the datasets that we study where high coverage can lead to low distributional shift during offline RL. We provide intuitions on why UDS works or does not work under each scenario and refer to the cases shown in our analysis in Section~\ref{sec:uds_theory}.}
\vspace{-0.43cm}
\begin{center}
\scriptsize
\resizebox{\textwidth}{!}{\begin{tabular}{l|r|l}
\toprule
 \textbf{Scenarios} & \textbf{UDS} & \textbf{Intuition} \\
 \midrule
  \textbf{L}: limited + high-quality + narrow, \textbf{U}: abundant + low/medium-quality + broad & \textcolor{green}{\checkmark} & increase coverage (case \textbf{\rom{2}} and \textbf{\rom{3}})\\
  \textbf{L}: limited + medium-quality + narrow, \textbf{U}: \ak{abundant} + low/medium-quality + broad &  \textcolor{red}{$\times$} & reward bias outweighs high coverage\\
  \textbf{L}: limited + high-quality + narrow, \textbf{U}: abundant + high-quality + narrow &   \textcolor{green}{\checkmark} & identical distribution (case \textbf{\rom{1}})\\
  \textbf{L}: limited + low-quality + narrow, \textbf{U}: abundant + high-quality + narrow & \textcolor{green}{\checkmark} & increase data quality (case \textbf{\rom{2}})\\
\bottomrule
\end{tabular}}
\end{center}
\vspace{-0.7cm}
\label{tbl:summary_criteria}
\normalsize
\end{table*}

\begin{theorem}[\textbf{Policy improvement guarantee for UDS}] 
\label{prop:uds_ours}
Let $\pi^*_\text{UDS}$ denote the policy learned by UDS, and let $\pi^\mathrm{eff}_\beta(\ba|\bs)$ denote the behavior policy for the combined dataset $\mathcal{D}^\mathrm{eff}$. Then with high probability $\geq 1 - \delta$, $\pi^*_\text{UDS}$ is a safe policy improvement over $\pi_\beta^\mathrm{eff}$, i.e.,
\begin{align*}
& J(\pi^*_\text{UDS}) \geq J(\pi_\beta^\mathrm{eff}) - \zeta_\text{err} +  \underbrace{\frac{\alpha}{1 - \gamma} D(\pi^*_\text{UDS}, \pi^\mathrm{eff}_\beta)}_{\text{(c): policy improvement}},\\
 & \zeta_\text{err} = \underbrace{\mathrm{RewardBias}(\pi^*_\text{UDS}, \pi^\mathrm{eff}_\beta)}_{ \text{(a)}} \\
 &+\underbrace{\mathcal{O}\left(\frac{\gamma}{(1 - \gamma)^2}\right) \mathbb{E}_{\bs, \ba \sim \widehat{d}^{\pi}}\left[\sqrt{\frac{D_{\text{CQL}}(\pi^*_\text{UDS}, \pi^\mathrm{eff}_\beta)(\bs)}{|\mathcal{D}^\mathrm{eff}(\bs)|}} \right]}_{\text{(b): sampling error}},\\
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!(a) &:= \frac{\sum_{\bs, \ba}\Delta\left(\widehat{d}^{\behavior^\mathrm{eff}}, \widehat{d}^{\pi^*_\text{UDS}}\right)  \cdot (1 - f(\bs, \ba)) \cdot r(\bs, \ba)}{1 - \gamma},
\end{align*}
where we use the notation $f(\bs, \ba) := \frac{|\mathcal{D}_\mathrm{L}(\bs, \ba)|}{|\mathcal{D}^\mathrm{eff} (\bs, \ba)|}$ and $\Delta(\widehat{d}^{\behavior^\mathrm{eff}}, \widehat{d}^{\pi^*_\text{UDS}}) = \widehat{d}^{\behavior^\mathrm{eff}}(\bs, \ba) - \widehat{d}^{\pi^*_\text{UDS}}(\bs, \ba)$. 
\end{theorem}
A proof for Theorem~\ref{prop:uds_ours} is provided in Appendix~\ref{proof:uds_proof}. Intuitively, term (a) corresponds to the potential suboptimality incurred as a result of using the wrong reward, term (b) corresponds to the suboptimality induced due to sampling error. Finally, term (c) corresponds to the policy improvement in the empirical MDP induced by the transitions in $\mathcal{D}^\mathrm{eff}$ that occurs as a result of offline RL. Intuitively, we expect that including more unlabeled data will reduce the sampling error (b) and potentially increase how much we can improve the policy (c), while potentially increasing the reward bias term (a). The key question is under which conditions we would expect the increase in bias (a) to be lower than the decrease in term (b) obtained from using the unlabeled data. We examine this question below, presenting a few common cases where we expect this tradeoff to be favorable.

\textbf{(\rom{1}) Unlabeled data is distributed identically as labeled data.} The first special case we consider is when the distribution of state-action pairs in $\mathcal{D}_\mathrm{L}$ is {identical} to the distribution of state-action pairs in the unlabeled dataset $\mathcal{D}_U$. This can arise in many application domains, such as in robotics~\citep{xie2019improvisation,dasari2020robonet}, where a large amount of offline data is available, but only a limited uniformly-selected fraction of it can be annotated with rewards. In this case, the fraction $f(\bs, \ba)$ takes on identical values for all state-action pairs, and term (a) simply reverts to be a difference between the performance of the effective behavior policy and the learned policy, in the empirical MDP. Since offline RL algorithms would improve over the effective behavior policy in the empirical MDP, this term is negative and hence, no additional suboptimality is incurred in the reward bias term. Moreover, the sampling error term \final{(b)} reduces when more data is utilized. Thus, in this case, \uds\ improves performance due to an increase in the dataset size $|\mathcal{D}^\mathrm{eff}(\bs)|$, without incurring a cost due to the wrong reward.   

\textbf{(\rom{2}) Quality of the unlabeled dataset.} In practice, we are often provided with a small amount of high-quality reward annotated demonstration data, and a lot of unlabeled prior data of low or mediocre quality. In this case, assigning a low reward to the transitions in the unlabeled dataset does not negatively affect policy performance significantly because the bias due to wrong reward is low (due to low-quality of labeled data) and reduces sampling error (term \final{(b)}). On the other hand, when the unlabeled data is of high quality and large in size compared to the labeled dataset, even then the performance of the policy $J(\pi^*_{\mathrm{UDS}})$ can be improved by using this unlabeled set since \uds\ improves $J(\pi_\beta^\mathrm{eff})$. 

\textbf{(\rom{3}) Large unlabeled datasets for long-horizon tasks.} Another scenario when \uds\ relabeling will be beneficial to do compared to not using the unlabeled data at all is in long-horizon tasks (large value of $1/(1 - \gamma)$), where a lot of unlabeled data is available, while the labeled dataset, $\mathcal{D}_\mathrm{U}$ is relatively very small. Define  $H = \frac{1}{1 - \gamma}$; then in the case that $|\mathcal{D}^\mathrm{eff}(\bs)| = \Omega(H^2) |\mathcal{D}_\mathrm{L}(\bs)|$, the sampling error term (term \final{(b)}) will consist of one less factor of $1/(1 - \gamma)$ when utilizing unlabeled data, compared to when it is not. Since the sampling error grows quadratically in the horizon, whereas the reward bias only grow linearly, a reduction in this term by increasing $|\mathcal{D}^\mathrm{eff}(\bs)|$ (i.e., denominator) can improve compared to only using the labeled data, $\mathcal{D}_\mathrm{L}$. Thus, even though the rewards may be biased, the addition of large amounts of unlabeled, diverse data in long-horizon tasks can help despite the reward bias incurred. 

We empirically verify that \uds\ indeed helps in the special cases discussed above in Section~\ref{sec:empirical_analysis}. However, there are also cases where \uds\ does not help because of large suboptimality induced due to term (a). In Table \ref{tbl:summary_criteria}, we present a summary of the scenarios under which we expect \uds\ will help or hurt performance.
As an example of the latter, when the amount of unlabeled data, $\mathcal{D}_\mathrm{U}$ is not very large compared to the labeled dataset, such that a decrease in sampling error does not outweigh the suboptimality induced by reward bias, we should not expect \uds\ to attain very good performance, which we empirically show in Appendix~\ref{app:unlabeled_dataset_size_analysis}. To handle such cases, our key idea is to re-weight the unlabeled dataset before using it for offline RL training reduce the sampling error and reward bias.

\vspace{-0.05cm}
\subsection{Reducing Reward Bias by Reweighting Data}
\label{sec:rebalancing}
\vspace{-0.05cm}
As discussed above, one way to reduce the suboptimality induced due to reward bias is by preferentially reweighting transitions in the unlabeled data. We would hope that such a scheme can provide a favorable bias-sampling error tradeoff, even though it reduces sample size. In this section, we will derive an optimized reweighting scheme that attains a favorable tradeoff. \ak{Intuitively, this optimized scheme suggests that reweighting must reduce distributional shift against the state-action marginal of the policy obtained by running offline RL on only the transitions in the labeled data.}
This scheme intuitively matches the conservative data sharing method~\citet{yu2021conservative} previously proposed for (fully-labeled) multi-task offline RL. We will show that this conservative sharing approach reduces reward bias, controls distributional shift that appears in the numerator of sampling error, and increases the sample size.   

Formally, we will derive this reweighting scheme from the perspective of optimizing the effective behavior policy, $\pi^\mathrm{eff}_\beta$ induced by the dataset $\mathcal{D}$ after preferentially sharing transitions from the unlabeled data, so as to minimize reward bias and sampling error, while improving the dataset quality. For understanding purposes, we begin by deriving the choice of $\pi^\mathrm{eff}_\beta$ that reduces only the reward bias component:
\begin{theorem}[\textbf{Optimized reward bias reduction}] 
\label{prop:reward_bias_theorem}
The optimal effective behavior policy that minimizes the bias (a) in Theorem~\ref{prop:uds_ours}, $\mathrm{RewardBias}(\pi, \pi^\mathrm{eff}_\beta)$, satisfies
\begin{align*}
    \widehat{d}^{\widehat{\pi}^\mathrm{eff}_\beta}(\bs, \ba) \propto  \sqrt{{d}_\mathrm{L}(\bs, \ba) d^{\pi}(\bs, \ba)},
\end{align*}
where $d^{\pi}$ denotes the state-action marginal of a policy $\pi$, and $d_\mathrm{L}(\bs, \ba)$ denotes the density of state-action pair $(\bs, \ba)$ under the labeled dataset.
\end{theorem}
A proof of Theorem~\ref{prop:reward_bias_theorem} is provided in Appendix~\ref{sec:small_reward_bias}. The expression implies that the state-action marginal of the effective behavior policy (i.e., the rebalanced dataset distribution) must place mass on state-action tuples that are both likely to under the learned policy $d^{\pi}$ and appear frequently in the distribution induced by the labeled dataset $\widehat{d}_\mathrm{L}$. However, note that Theorem~\ref{prop:reward_bias_theorem} only accounts for the reward bias and not the other terms pertaining to sampling error and the performance of the effective behavior policy that appear in Theorem~\ref{prop:uds_ours}. To address both of these issues, in our next theoretical result, Theorem~\ref{thm:with_all_sources}, we derive the reweighting distribution that controls all the terms.
\begin{theorem}[\textbf{Optimized reweighting unlabeled data}; Informal]
\label{thm:with_all_sources}
The optimal effective behavior policy that maximizes a lower bound on $J(\pi_\beta^\mathrm{eff}) - \left[(a) + (b)\right]$ in Theorem~\ref{prop:uds_ours} satisfies $d^{\widehat{\pi}_\beta^\mathrm{eff}}(\bs, \ba) = p^*(\bs, \ba)$, where:
\begin{align*}
    p^* = \arg\min_{p \in \Delta^{|\mathcal{S}||\mathcal{A}|}}&~ \sum_{\bs, \ba} C_1 \frac{\widehat{d}^\pi(\bs, \ba)}{\sqrt{p(\bs, \ba)}} + C_2 |\widehat{d}_\mathrm{L}(\bs, \ba)| \frac{\widehat{d}^\pi(\bs, \ba)}{p(\bs, \ba)}, 
\end{align*}
where $C_1$ and $C_2$ are universal positive constants that depend on the sizes of the labeled and unlabeled datasets.
\end{theorem}
A proof of Theorem~\ref{thm:with_all_sources} along with a more formal statement listing the constants $C_1$ and $C_2$ is provided in in {Appendix~\ref{proof:all_sources}}. The first term in the optimization objective of $p^*$ appearing above arises from the sampling error term, while the second term corresponds to the reward bias term in Theorem~\ref{prop:uds_ours}. The optimal solution for $p^*$ must place high density on $(\bs, \ba)$ pairs where $\widehat{d}^\pi(\bs, \ba)$ is high, because this would reduce the objective in the optimization problem above. This corroborates the analysis of \citet{yu2021conservative}, which shows that utilizing a reweighting scheme that reduces distributional shift (i.e., makes $\pi(\ba|\bs)/\widehat{\pi}^\mathrm{eff}_\beta(\ba|\bs)$ or \ak{equivalently}, as we find, making $\widehat{d}^\pi(\bs, \ba)/\widehat{d}^{\pi_\beta^\mathrm{eff}}(\bs, \ba)$ smaller) will control sampling error, and give rise to performance benefits. In addition, as also shown in Theorem~\ref{prop:reward_bias_theorem}, the reward bias term is also controlled when low distributional shift appears. This means that rebalancing the dataset to control distributional shift between the learned policy $\widehat{d}^\pi(\bs, \ba)$ and $\widehat{d}^{\pi^\mathrm{eff}_\beta}(\bs, \ba)$ is effective in unlabeled settings as well.


\begin{table*}[t]
\vspace{-0.2cm}
\caption{\footnotesize Results on single-task environments {hopper} and {AntMaze} from the D4RL~\citep{fu2020d4rl} benchmark. The numbers are averaged over three random seeds. We only bold the best-performing method that does not have access to the true reward for relabeling. UDS outperforms No Sharing in three out of the four settings while achieving competitive performances compared to Sharing All in all the settings. CDS+UDS further improves over UDS in three out of four settings.}
\vspace{-0.24cm}
\begin{center}
\resizebox{\textwidth}{!}{\begin{tabular}{l|l|l|rrrrrr|rr}
\toprule
& & & & & & & & & \multicolumn{2}{c}{\textbf{Oracle Methods}} \\
 \textbf{Environment} & \textbf{Labeled data} & \textbf{Unlabeled data}   & \textbf{CDS+UDS}   & \textbf{UDS}         & \textbf{No Sharing} & \textbf{Reward Pred.} & \textbf{VICE} & \textbf{RCE}  & \textbf{CDS} & \textbf{Sharing All} \\
 \midrule
 D4RL hopper & expert & random & \textbf{81.5}  & 78.6 & 77.1 & 67.6 & n/a & n/a & 83.3 & 86.1\\
  & expert & medium & \textbf{78.3}  & 64.4 & 77.1 & 51.7 & n/a & n/a & 82.5 & 64.6\\
\midrule
D4RL AntMaze & expert & medium-play & 82.6  & \textbf{82.7} & 17.2 & 0.0 & 0.0 & 0.0 & 83.5 & 83.1 \\
 & expert & large-play & \textbf{47.1} & 33.1 & 0.7 & 0.0 & 0.0 & 0.0 & 46.1 & 50.2\\
\bottomrule
\end{tabular}}
\end{center}
\vspace{-0.7cm}
\label{tbl:single_task}
\normalsize
\end{table*}

While the scheme derived above can, in principle, be implemented exactly in practice, it would require computing state-marginals. Since, computing state marginals accurately in an offline setting has been an outstanding challenge,
we instead can utilize a reweighting scheme that corrects for distributional shift approximately without needing state-marginals. One of such methods is conservative data sharing (CDS)~\citep{yu2021conservative} that can be implemented without requiring additional components beyond the machinery of the offline RL method. Formally, CDS is given by:
\begin{equation*}
    \mathcal{D}^\mathrm{eff}_i = \mathcal{D}_i \cup ( \cup_{j \neq i}\{(\bs_j, \ba_j, \bs'_j, r_i) \in \mathcal{D}_{j \rightarrow i}: \Delta^\pi(\bs, \ba) \geq 0\}),
\end{equation*}
where $\bs_j, \ba_j, \bs'_j$ denote the transition from $\mathcal{D}_j$, $r_i$ denotes the reward of $\bs_j, \ba_j, \bs'_j$ relabeled for task $i$, $\pi$ denotes the task-conditioned policy $\pi(\cdot|\cdot, i)$, $\Delta^\pi(\bs_j, \ba_j)$ is the condition that shares data only if the expected conservative Q-value of the relabeled transition exceeds the top $k$-percentile of the conservative Q-values of the original data. In our experiments and analysis in Section \ref{sec:exp}, we find that utilizing CDS improves performance over simply training with \uds\ in a number of domains supporting the theoretical analysis. 


\subsection{Why Can We Expect UDS to Outperform Reward Prediction Methods?}
\label{sec:reward_predictor_discussion}
While we have discussed various conditions where we would expect UDS (with or without various reweighting methods) to improve final performance over an approach that does not utilize the unlabeled data, it is also instructive to consider how it comes to a method that instead trains an approximate reward function, $\widehat{r}_\phi(\bs, \ba)$ using the labeled data, and then uses this approximate reward to annotate the unlabeled data. In our experiments, we will show, perhaps surprisingly that UDS often outperforms prior reward learning methods. In this section, we provide some intuition for why. 
First, we note the following generic expression for reward bias (term (a) in Theorem~\ref{prop:uds_ours}) for any approach:
\begin{align*}
    \mathrm{RewardBias}(\pi, \pi^\mathrm{eff}_\beta) = \frac{\sum_{\bs, \ba} \Delta\left(\widehat{d}^{\behavior^\mathrm{eff}}, \widehat{d}^{\pi}\right) \cdot \Delta r(\bs, \ba)}{1 - \gamma},
\end{align*}
where $\Delta r(\bs, \ba)$ is the error in the reward applied to the unlabeled data, such that $\Delta r(\bs, \ba) = (1 - f(\bs, \ba)) r(\bs, \ba)$ for UDS, and $\Delta r(\bs, \ba) = r(\bs, \ba) - \widehat{r}_\phi(\bs, \ba)$ for a reward prediction method. Note that while for UDS, $\forall~\bs, \ba, ~\Delta r(\bs, \ba) \geq 0$, this is not necessarily the case for a generic reward prediction method.

\textbf{UDS.} Since $\Delta r(\bs, \ba) \geq 0$ for all state-action tuples, state-action pairs that appear more frequently under the learned policy compared to the effective behavior policy, i.e., when $\Delta\left(\widehat{d}^{\behavior^\mathrm{eff}}, \widehat{d}^{\pi}\right) < 0$, contribute to reducing the suboptimality induced due to reward bias. 

\textbf{Reward prediction.} When $\Delta r(\bs, \ba) = r(\bs, \ba) - \widehat{r}_\phi(\bs, \ba)$, $\Delta r(\bs, \ba)$ may not be positive on all state-action tuples, and thus reward prediction methods fail to reduce the contribution of such state-action pairs in term (a). Since policy optimization will seek out those policies that maximize $\widehat{d}^\pi(\bs, \ba)$ on state-action pairs with high rewards, state-action pairs where $\Delta(\widehat{d}^{\pi_\beta^\mathrm{eff}}, \widehat{d}^\pi) < 0$ (i.e., state-action pairs that appear more under the learned policy) are likely to also have $\Delta r(\bs, \ba) < 0$. This ``exploitation'' inhibits the correction of reward bias and provides an explanation for why reward prediction approaches may still not perform well due to overestimation errors in the reward function.  

==> UDS_ICML_camera_ready_arXiv 2/prelim.tex <==
\section{Preliminaries}
\vspace{-0.15cm}
\label{sec:prelim}

\textbf{Offline RL.} Standard RL considers a Markov decision process (MDP), $\mdp =(\states, \actions, P, \gamma, R)$, where $\states$ and $\actions$ denote the state and action spaces respectively, $P(\bs' | \bs, \ba)$ denotes the dynamics, $\gamma \in [0, 1)$ is the discount factor, and $R$ correspond to the reward function. Offline RL tackles the problem of learning a policy $\pi(\ba|\bs)$ from a static dataset with $\mathcal{D}$, generated by a behavior policy $\pi_\beta(\ba|\bs)$.


\textbf{Data sharing in offline RL.} Data sharing has been considered in the multi-task offline RL setting where there is a static multi-task dataset with $\mathcal{D} = \cup_{i=1}^N \mathcal{D}_i$ where $N$ is the number of tasks. Prior works~\citep{kalashnikov2021mt,eysenbach2020rewriting,yu2021conservative} show that sharing data from different tasks to task $i$ to be conducive. To do so, these prior methods assume access to the functional form of the reward $r_i$. This is a strong assumption in practice, as it necessitates access to a functional (programmatic) form for the reward function. In offline RL, it might be desirable to simply label the reward function by hand, but then the algorithm does not have access to the functional form of the reward, and all unlabeled data also needs to be labeled by hand for use with such methods. Our aim in this paper is to utilize unlabeled data without any reward labels at all.
If however functional access to the reward \emph{is} available, a simple strategy is to na\"ively share data across all tasks, which we refer to as Sharing All. Formally, Sharing All defines the dataset of transitions relabeled from task $j$ to task $i$ as $\mathcal{D}_{j \rightarrow i}$ and the method can be then defined as
    $\mathcal{D}^\mathrm{eff}_i := \mathcal{D}_i \cup ( \cup_{j \neq i} \mathcal{D}_{j \rightarrow i})$,
where $\mathcal{D}^\mathrm{eff}_i$ denotes the effective dataset for task $i$. Therefore, the policy optimization objective in Sharing All can be written as follows:
\begin{equation*}
     \forall i \in [N], ~~\pi^*(\ba|\bs, i) := \arg \max_{\pi}~~ J_{\mathcal{D}^\mathrm{eff}_i}(\pi) - \alpha D(\pi, \pi^\mathrm{eff}_\beta),
\end{equation*}
where $\pi_\beta^\mathrm{eff}(\ba|\bs, i)$ is the effective behavior policy for task $i$ denoted as $\pi_\beta^\mathrm{eff}(\ba|\bs, i) := |\mathcal{D}^\mathrm{eff}_i(\bs, \ba)| / |\mathcal{D}^\mathrm{eff}_i(\bs)|$, $J_{\mathcal{D}^\mathrm{eff}_i}(\pi)$ denotes the average return of policy $\pi$ in the empirical MDP induced by the effective dataset, and $D(\pi, \pi^\mathrm{eff}_\beta)$ denotes a divergence measure (e.g., KL-divergence~\citep{jaques2019way,wu2019behavior}, fisher divergence~\citep{kostrikov2021offline}, MMD distance~\citep{kumar2019stabilizing} or $D_{\text{CQL}}$ from conservative Q-values~\citep{kumar2020conservative}) between the learned policy $\pi$ and the effective behavior policy $\pi_\beta^\mathrm{eff}$. Note that conservative Q-values refer to the Q-value for a given policy corresponding to a modified reward function $r(\bs, \ba) - \alpha \pi(\ba|\bs) \cdot (\pi(\ba|\bs) / \pi_\beta(\ba|\bs) - 1)$, computed on the empirical MDP. We also note that Sharing All can be easily adapted to the single-task setting where there is only one target task with labeled data $\mathcal{D}_\text{L}$ and unlabeled prior data $\mathcal{D}_\text{U}$. While data sharing tends to show promising results, it requires the assumption of the access to the functional form of the reward function. We instead focus on the data sharing problem where we do not make such an assumption and instead, only have the reward labels for originally commanded task, which we will discuss in the following section.




==> UDS_ICML_camera_ready_arXiv 2/related_work.tex <==
\section{Related Work}

\textbf{Offline RL.} Offline RL~\citep{ernst2005tree,riedmiller2005neural,LangeGR12,levine2020offline} considers the problem of learning a policy from a static dataset without interacting with the environment, which has shown promises in many practical applications such as robotic control~\citep{kalashnikov2018scalable,Rafailov2020LOMPO}, NLP~\citep{jaques2019way}, 
and healthcare~\citep{shortreed2011informing, Wang2018SupervisedRL}. 
The main challenge of offline RL is the distributional shift between the learned policy and the behavior policy~\citep{fujimoto2018off}, which can cause erroneous value backups. To address this issue, prior methods have constrained the learned policy to be close to the behavior policy via policy regularization~\citep{liu2020provably,wu2019behavior,kumar2019stabilizing, zhou2020plas,ghasemipour2021emaq,fujimoto2021minimalist}, conservative value functions~\citep{kumar2020conservative}, 
and model-based training with conservative penalties~\citep{yu2020mopo,kidambi2020morel,swazinna2020overcoming,lee2021representation,yu2021combo}. Unlike these prior works, we study how unlabeled data can be incorporated into the offline RL framework.

\textbf{RL with unlabeled data.} Prior works tackle the problem of learning from data without reward labels via either directly imitating expert trajectories~\citep{pomerleau1988alvinn,RossB12,GAIL2016Ho}, learning reward functions from expert data using inverse RL~\citep{abbeel2004apprenticeship,ng2000irl,ziebart2008maximum,finn2016guided,AIRLFu2018,konyushkova2020semi}, or learning a reward / value classifier that discriminates successes and failures~\citep{xie2018few,VICEFu2018,singh2019end,eysenbach2021replacing} in standard online RL settings. 
{Unlike these prior works, the goal of our paper is not to propose a sophisticated new algorithm for reward learning,} but rather to study when the simple solution of using zero as the reward label can work well from offline data. \final{While} \citet{singh2020cog} also considers relabeling prior data with zero reward in the standard, single-task offline RL setting, \final{the key distinction is that the unlabeled data in \citet{singh2020cog} cannot solve the target task and \emph{actually} gets zero rewards and is thus labeled with the true reward. Unlike \citet{singh2020cog}, we show that UDS can surprisingly also be effective even when the unlabeled data is incorrectly labeled with zero reward, and discuss how it can be improved (Section~\ref{sec:rebalancing}).}
Additionally, we consider both single-task and multi-task offline RL settings.

\textbf{Data sharing.} 
Sharing data across different tasks has been found to be effective in multi-task~\citep{eysenbach2020rewriting,kalashnikov2021mt,yu2021conservative} and meta-RL~\citep{dorfman2021offline,mitchell2021offline} and it improves performance significantly in multi-task offline RL. 
Prior works share data based on learned Q-values~\citep{eysenbach2020rewriting,li2020generalized,yu2021conservative}, domain knowledge~\citep{kalashnikov2021mt} and distance to goals in goal-conditioned settings~\citep{andrychowicz2017hindsight,liu2019competitive,sun2019policy,lin2019reinforcement,chebotar2021actionable}, and the learned distance with robust inference in the offline meta-RL setting~\citep{li2019multi}. However, all of these either require access to the functional form of the reward for relabling or are limited to goal-conditioned settings. In contrast, we attempt to tackle a more general problem where reward labels are not provided for a subset of the data, either in a  multi-task or a single-task setting and find that simple approaches for relabeling data from other tasks with the constant zero can work well. 


==> intro.tex <==
\section{Introduction}
